Quantum Generative Models for Image Generation: Insights from MNIST and MedMNIST

Quantum generative models offer a promising new direction in machine learning by leveraging quantum circuits to enhance data generation capabilities. In this study, we propose a hybrid quantum-classical image generation framework that integrates variational quantum circuits into a diffusion-based model. To improve training dynamics and generation quality, we introduce two novel noise strategies: intrinsic quantum-generated noise and a tailored noise scheduling mechanism. Our method is built upon a lightweight U-Net architecture, with the quantum layer embedded in the bottleneck module to isolate its effect. We evaluate our model on MNIST and MedMNIST datasets to examine its feasibility and performance. Notably, our results reveal that under limited data conditions (fewer than 100 training images), the quantum-enhanced model generates images with higher perceptual quality and distributional similarity than its classical counterpart using the same architecture. While the quantum model shows advantages on grayscale data such as MNIST, its performance is more nuanced on complex, color-rich datasets like PathMNIST. These findings highlight both the potential and current limitations of quantum generative models and lay the groundwork for future developments in low-resource and biomedical image generation.

==> sections/abstract.tex <==
Quantum machine learning has recently attracted considerable attention due to its potential to surpass classical approaches in specific computational tasks. In particular, quantum generative models, which utilize quantum mechanical phenomena to enhance generative capabilities, are gaining traction. Variational quantum circuits (VQCs), a prominent class of quantum algorithms, offer a promising approach for building these generative models, especially for image generation tasks. Our method is assessed through two representative datasets: MNIST, widely recognized as a standard benchmark for handwritten digit recognition, and MedMNIST, a suite of medical imaging datasets aimed at benchmarking machine learning tasks in healthcare. By integrating hybrid quantum-classical optimization techniques, our model addresses current limitations inherent in quantum hardware, making it feasible for practical use. Experimental evaluations indicate our quantum generative model achieves performance levels comparable to current classical generative methods. We further investigate how quantum entanglement and circuit depth affect generative performance, providing insights into scalability and improvements for broader applications.



==> sections/discussion.tex <==
% The results from our experiments provide a number of insights into the capabilities and current limitations of quantum generative models on image data. First, the \textbf{performance gap between the quantum model and classical benchmarks} highlights the challenges faced by quantum networks with limited size. Our 4-qubit generator was able to learn coarse features of digit images, but struggled with finer details and diversity. This is partly due to the low effective dimensionality of the model’s output space—with only 4 qubits, even if each could produce a continuous value, the model has far fewer degrees of freedom than a typical classical generator neural network. Increasing the qubit count could exponentially enlarge the state space, but current hardware restricts us to only a handful of qubits with reliable operation. Additionally, the necessity to measure quantum states to obtain outputs inherently introduces sampling noise and collapses the rich superposition to a few samples per run, reducing the information throughput to the discriminator.

% Another critical factor is \textbf{circuit depth and expressivity}. We found that a shallow circuit (1–2 layers) was insufficient to generate meaningful images, while a deeper circuit improved results up to a point. However, beyond a certain depth, training became unstable or plateaued. This behavior is reminiscent of the “barren plateau” problem in training deep quantum circuits, where gradients vanish as circuit depth increases, hindering learning. Noise on real quantum hardware would exacerbate this issue: our simulations assumed an ideal noiseless quantum environment, but in practice, gate errors and decoherence would degrade the output quality. Thus, there is a trade-off between making the circuit expressive enough to model the data distribution and keeping it shallow/simple enough to train on NISQ devices. Techniques like parameter initialization strategies or layer-wise training could mitigate these training difficulties but were beyond the scope of our current implementation.

% The \textbf{hybrid training process} also influenced model quality. Using a classical discriminator to guide the quantum generator proved effective, but we observed that the discriminator can sometimes overpower the generator early in training (a common GAN issue). In our runs, we occasionally paused discriminator training to give the quantum generator more opportunity to catch up. This points to the need for careful tuning of the training loop, or possibly more advanced loss functions (e.g., Wasserstein loss with gradient penalty) to stabilize the adversarial training involving quantum components. Interestingly, when the model did train successfully, the feedback from the classical network allowed the quantum circuit to gradually adjust its parameters in the right direction. This underscores that current hybrid approaches are viable: quantum circuits can be treated as differentiable modules within a larger classical training framework, as facilitated by tools like PennyLane, and they can be trained with gradient-based methods despite the underlying quantum complexity.

% One surprising observation was that the quantum generator, even with very few parameters, sometimes achieved a comparable level of performance to a classical GAN with orders of magnitude more parameters, particularly on the constrained MNIST task. This result aligns with recent findings indicating the potential of quantum circuits to efficiently represent certain probability distributions~\cite{rudolph2024quantum}. The entanglement inherent in quantum states might enable compact encoding of pixel correlations, which otherwise could require substantially larger classical layers to replicate~\cite{anschuetz2023interpretable}. However, this quantum advantage remained modest in our case, accompanied by higher output variance and greater training difficulties. Whether scaling the quantum model (increasing qubits with controlled noise) would significantly amplify this advantage or merely achieve parity with classical performance remains an open research question.

% Current quantum hardware limitations heavily impacted our design choices. With only simulation, we did not encounter real noise, but we did restrict qubit count and circuit depth to what near-term devices might handle (e.g., 4 qubits, 3 layers). If we were to deploy on an actual quantum processor, gate errors would likely blur the generated images significantly. Error mitigation techniques could be necessary to get clear outputs. Additionally, the requirement of many repeated measurements (shots) to build up an image sample is time-consuming on hardware. In the future, \textbf{improvements in quantum hardware}—such as higher qubit counts, lower error rates, and faster sampling—will directly translate to better generative model performance. It will be important to test this model on hardware as devices progress to identify any unforeseen issues in the quantum-classical interface (for example, readout errors affecting the discriminator’s feedback).

% Finally, we discuss the \textbf{implications for quantum advantage in generative modeling}. Although our study did not conclusively demonstrate quantum advantage, it provides foundational insights and clearly identifies current bottlenecks. Achieving quantum advantage likely requires targeting problems where classical models inherently struggle yet quantum circuits can naturally encode complex solutions~\cite{anschuetz2023interpretable}. For instance, quantum models may excel in capturing high-dimensional distributions with intricate entanglement structures, potentially enabling efficient representation of global image properties. Encouragingly, despite significant hardware constraints, our quantum model successfully learned recognizable visual patterns. Continued hardware improvements, enhanced training methodologies, and strategic hybrid quantum-classical approaches—such as leveraging classical autoencoders for dimensionality reduction prior to quantum generation—will be crucial for unlocking genuine quantum advantage~\cite{rudolph2024quantum,khatun2023quantum}. These results offer a clear roadmap and practical starting points for future exploration into quantum-enhanced generative modeling.

